Benford-Newcomb Subsequences for Fraud Detection

Benford's law is frequently used to evaluate the likihood that data is misrepresentative. Typically statistical tests measure the likihood. Another method of employing Benford's law is to compare the frequency of leading digits to the probabilities of leading digits over a subset of the natural numbers. This paper proposes using the probabilities of leading digits from uniform, natural numbers to establish interval criteria for when to look more closely into the possibility of misrepresentative data.

==> BenfordSubsequenceBibtex.tex <==
@article{benford1938law,
  title={The law of anomalous numbers},
  author={Benford, F.},
  journal={Proceedings of the American Philosophical Society},
  pages={551--572},
  year={1938},
  publisher={JSTOR}
}

@article {MR1505286,
    AUTHOR = {Newcomb, Simon},
     TITLE = {Note on the {F}requency of {U}se of the {D}ifferent {D}igits
              in {N}atural {N}umbers},
   JOURNAL = {Amer. J. Math.},
  FJOURNAL = {American Journal of Mathematics},
    VOLUME = {4},
      YEAR = {1881},
    NUMBER = {1-4},
     PAGES = {39--40},
      ISSN = {0002-9327},
     CODEN = {AJMAAN},
   MRCLASS = {Contributed Item},
  MRNUMBER = {1505286},
       DOI = {10.2307/2369148},
       URL = {http://dx.doi.org/10.2307/2369148},
}

@article {MR1421567,
    AUTHOR = {Hill, Theodore P.},
     TITLE = {A statistical derivation of the significant-digit law},
   JOURNAL = {Statist. Sci.},
  FJOURNAL = {Statistical Science. A Review Journal of the Institute of
              Mathematical Statistics},
    VOLUME = {10},
      YEAR = {1995},
    NUMBER = {4},
     PAGES = {354--363},
      ISSN = {0883-4237},
   MRCLASS = {60E99 (60A10 62E99)},
  MRNUMBER = {1421567 (98a:60021)},
MRREVIEWER = {Peter Schatte},
       URL =
              {http://links.jstor.org/sici?sici=0883-4237(199511)10:4<354:ASDOTS>2.0.CO;2-P&origin=MSN},
}

@Manual{RCoreTeam,
    title = {R: A Language and Environment for Statistical Computing},
    author = {{R Core Team}},
    organization = {R Foundation for Statistical Computing},
    address = {Vienna, Austria},
    year = {2012},
    note = {{ISBN} 3-900051-07-0},
    url = {http://www.R-project.org/},
  }
